Averaging Spatio-temporal Signals using Optimal Transport and Soft Alignments

Several fields in science, from genomics to neuroimaging, require monitoring populations (measures) that evolve with time. These complex datasets, describing dynamics with both time and spatial components, pose new challenges for data analysis. We propose in this work a new framework to carry out averaging of these datasets, with the goal of synthesizing a representative template trajectory from multiple trajectories. We show that this requires addressing three sources of invariance: shifts in time, space, and total population size (or mass/amplitude). Here we draw inspiration from dynamic time warping (DTW), optimal transport (OT) theory and its unbalanced extension (UOT) to propose a criterion that can address all three issues. This proposal leverages a smooth formulation of DTW (Soft-DTW) that is shown to capture temporal shifts, and UOT to handle both variations in space and size. Our proposed loss can be used to define spatio-temporal barycenters as Fr\'echet means. Using Fenchel duality, we show how these barycenters can be computed efficiently, in parallel, via a novel variant of entropy-regularized debiased UOT. Experiments on handwritten letters and brain imaging data confirm our theoretical findings and illustrate the effectiveness of the proposed loss for spatio-temporal data.

==> ex_shared_siam.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Spatio-temporal barycenters}{H. Janati, M. Cuturi, A. Gramfort}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Spatio-temporal barycenters\thanks{Submitted to the editors DATE.
\funding{This work was funded by
	the European Research Council Starting Grant SLAB
	ERC-YStG-676943 and a chaire d’excellence
	de l’IDEX Paris Saclay }}}

% Authors: full names plus addresses.
\author{Hicham Janati \thanks{Inria Saclay | ENSAE, Paris, France
  (\email{hicham.janati@inria.fr}).}
\and Marco Cuturi \thanks{Google Brain | ENSAE , Paris, France,
  (\email{cuturi@google.com})}
\and Alexandre Gramfort \thanks{Inria Saclay, Paris, France
	(\email{alexandre.gramfort@inria.fr}).}}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> sec/background.tex <==
% !TEX root = ../main.tex

\section{Soft-DTW barycenters through alternating optimization}
\label{s:soft-dtw}


\paragraph{Dynamic time warping}
Consider two multivariate time series $\bx \in \bbR^{p, T_1}$ and $\by \in \bbR^{p, T_2}$ with respective lengths $T_1, T_2$ and having observations in $\bbR^p$. DTW is defined through some pairwise distance matrix $\Delta(\bx, \by) \in \bbR^{T_1, T_2}$ between all their time points such that the cost of a given alignment function $\sigma: \intset{1, T_1} \to \intset{1, T_2}$ is equal to $\sum_{i=1}^{T_1} \Delta(\bx_i, \by_{\sigma(i)})$. To guarantee the preservation of the chronology of the data, $\sigma$ must be increasing and verify $\sigma(1) = 1$ and $\sigma(T_1) = T_2$. The resulting optimization problem is however better posed as a minimization of $\sum_{i=1}^{T_1}\sum_{j=1}^{T_2} A_{ij}\Delta(\bx_i, \by_j)$ over the set of binary alignments $A$ on the rectangular lattice $\intset{1, T_1} \times \intset{1, T_2}$ where no temporal back steps are allowed. This amounts to considering  binary matrices with a non-zero path linking the corners of the lattice $(1, 1)$ (upper left) and $(T_1, T_2)$ (bottom right) using $\rightarrow, \downarrow, \searrow $ steps exclusively~\citep{sakoe78}. The binary nature of this set makes the DTW loss non-differentiable which is a major limitation when DTW is used as a loss function. To circumvent this issue, several authors introduced regularized variants of DTW \citep{saigo04, cuturi11, cuturi17}. Instead of selecting \emph{the} minimum cost alignment, Global Alignment Kernels (GAK) for instance \citep{saigo04, cuturi11} compute a weighted cost of all possible alignments with a certain smoothing hyperparameter. Similarly, the soft-minimum generalization approach of \cite{cuturi17} -- called soft-DTW -- provides a similar framework to that of GAK where gradients can easily be computed used a backpropagation of Bellman's equation~\citep{bellman}.

\subsection{Soft Dynamic Time Warping}
\paragraph{Forward recursion}
Let $\bx = (\bx_1^\top, \dots, \bx_{T_1}^\top)^\top \in \bbR^{T_1, p}$ and $\by = (\by_1^\top, \dots, \by_{T_2}^\top)^\top \in \bbR^{T_2, p}$ be two time series of respective lengths $T_1, T_2$ and dimension $p$. The set of all feasible alignments in a $(T_1, T_2)$ rectangle is denoted by $\cA_{T_1, T_2}$. Given a pairwise distance matrix $\Delta(\bx, \by) \eqdef (\delta(\bx_i, \by_j))_{ij}$, soft-DTW is defined as:
%
\begin{equation}
    \label{eq:sdtw}
    \sdtw(\bx, \by; \Delta) = {\softmin}_{\beta}\{\langle \bA, \Delta(\bx, \by)\rangle, \bA \in \cA_{T_1, T_2}\} \enspace ,
\end{equation}
%
where the soft-minimum operator of a set $\cA$ with parameter $\beta$ is defined as:
%
\begin{equation}
    {\softmin}_{\beta}(\cA) =
    \left\{\begin{array}{ll}
        -\beta \log\left(\sum_{\cA} e^{- \nicefrac{a}{\beta}}\right) \text{\quad if } \beta > 0\\
        \min_{a \in \cA} a \text{\quad if } \beta = 0
        \end{array} \right.
\end{equation}

Figure~\ref{f:dtw-example} illustrates two time series of images and their cost matrix $\Delta$. The path from (1, 1) to (5, 6) is an example of a feasible alignement in $\cA_{5, 6}$.
When $\beta = 0$, the soft-minimum is a minimum and $\sdtw$ falls back to the classical DTW metric. Nevertheless, it can still be computed using the dynamic program of Algorithm \ref{a:dynamicprogram} with a soft-min instead of min operator. % It is important to notice that Algorithm~\ref{a:dynamicprogram} stores the whole intermediary alignment matrix $R$ which is needed for automatic differentiation.

\begin{figure}[t]
    \centering
	\includegraphics[width=0.7\linewidth, trim={1.cm 0 1.cm 0},clip]{img/rugby}
	\caption{Example of Dynamic time warping alignment between two time series of images given a pairwise distance matrix. \label{f:dtw-example}}
\end{figure}


\begin{algorithm}[t]
   \caption{BP recursion to compute $\sdtw$ \cite{cuturi17} \label{a:dynamicprogram}}
\begin{algorithmic}
   \STATE {\bfseries Input:}  data $\bx, \by$ soft-min parameter $\beta$ and distance function $\delta$ 
      \STATE {\bfseries Output:} $\sdtw(\bx, \by) = r_{T_1, T_2}$
    \STATE $r_{0,0} = 0; r_{0,j} = r_{i, 0} =\infty$ for $i \in \intset{T_1}$, $j \in \intset{T_2}$ 
    \FOR{$i=1$ {\bfseries to} $T_1$}
    \FOR{$j=1$ {\bfseries to} $T_2$}
    \STATE $r_{i,j} = \delta(\bx_i, \by_j)$ ${\softmin}_\beta(r_{i-1, j-1}, r_{i-1, j}, r_{i, j-1})$
      \ENDFOR
     \ENDFOR
\end{algorithmic}
\end{algorithm}

%
% \paragraph{Algorithmic differentiation}
% When $\beta > 0$, differentiating \eqref{eq:sdtw} with respect to $\bx$ yields:
% %
% \begin{equation}
%     \label{eq:gradient-sdtw}
%     \nabla_{\bx} \sdtw(\bx, \by, \Delta) = \left(\frac{\partial \Delta(\bx, \by)}{\partial \bx}\right)^\top E_{\beta}(\bx, \by) \enspace ,
% \end{equation}
% %
% where $E_{\beta}(\bx, \by) \eqdef \frac{\sum_{\cA_{T_1, T_2}} e^{-\frac{\langle \bA, \Delta(\bx, \by)\rangle}{\beta}} A}
%     {\sum_{\cA_{T_1, T_2}} e^{-\frac{\langle \bA, \Delta(\bx, \by)\rangle}{\beta}}}$.

% To compute $E_{\beta}(\bx, \by)$, \cite{cuturi17} propose to back propagate the forward recursion of Algorithm \ref{a:dynamicprogram}, starting from $E_{T_1, T_2}$ down to $E_{0. 0}$. Indeed, the value of $\sdtw$ is stored in the last alignment cost $r_{T_1,T_2}$. Thus differentiating $\sdtw$ with respect to any  $r_{i, j}$ only involves the terms of 
% $r_{i-1, j}, r_{i, j-1}$ and $r_{i-1, j-1}$. Differentiating the softmin operation of the forward pass yields the backward recursion of Algorithm \ref{a:backprop}.

% \begin{algorithm}
%   \caption{Backward recursion to differentiate sdtw.\label{a:backprop}}
% \begin{algorithmic}
%   \STATE {\bfseries Input:} $\bx, \by$, parameter $\beta$, distance $\delta$ and intermediary alignment matrix $R$
%       \STATE {\bfseries Output:} $E = E_\beta(\bx, \by)$
%     \STATE $r_{i,m+1} = r_{n+1,j} = -\infty$, $i \in \intset{n}$, $j \in \intset{m}$ 
%     \STATE $e_{i,m+1} = r_{n+1,j} = 0$, $i \in \intset{n}$, $j \in \intset{m}$ 
%     \STATE $\delta_{i,m+1} = \delta_{n+1,j} =0$, $i \in \intset{n}$, $j \in \intset{m}$ 
%     \STATE $\delta_{n+1,m+1} = 0, e_{n+1,m+1} =1, r_{n+1, m+1} = r_{n, m}$ 
%     \FOR{$i=1$ {\bfseries to} $n$}
%         \FOR{$j=1$ {\bfseries to} $m$}
%         \STATE $a = \exp \frac{1}{\beta}(r_{i+1, j} - r_{i, j} - \delta_{i+1, j})$
%         \STATE $b = \exp \frac{1}{\beta}(r_{i, j + 1} - r_{i, j} - \delta_{i, j + 1})$
%         \STATE $c = \exp \frac{1}{\beta}(r_{i+1, j+1} - r_{i, j} - \delta_{i+1, j+1})$
%         \STATE $e_{i,j} = a e_{i+1, j} + b e_{i, j+1} + c e_{i+1, j+1} $
%       \ENDFOR
%      \ENDFOR
% \end{algorithmic}
% \end{algorithm}

